A Review of Location Encoding for GeoAI: Methods and Applications

A common need for artificial intelligence models in the broader geoscience is to represent and encode various types of spatial data, such as points (e.g., points of interest), polylines (e.g., trajectories), polygons (e.g., administrative regions), graphs (e.g., transportation networks), or rasters (e.g., remote sensing images), in a hidden embedding space so that they can be readily incorporated into deep learning models. One fundamental step is to encode a single point location into an embedding space, such that this embedding is learning-friendly for downstream machine learning models such as support vector machines and neural networks. We call this process location encoding. However, there lacks a systematic review on the concept of location encoding, its potential applications, and key challenges that need to be addressed. This paper aims to fill this gap. We first provide a formal definition of location encoding, and discuss the necessity of location encoding for GeoAI research from a machine learning perspective. Next, we provide a comprehensive survey and discussion about the current landscape of location encoding research. We classify location encoding models into different categories based on their inputs and encoding methods, and compare them based on whether they are parametric, multi-scale, distance preserving, and direction aware. We demonstrate that existing location encoding models can be unified under a shared formulation framework. We also discuss the application of location encoding for different types of spatial data. Finally, we point out several challenges in location encoding research that need to be solved in the future.

==> application.tex <==
% \section{Where can we use Location Encoding?} 
\section{Different application domains for location encoding}
\label{sec:app}

%In this section, we will first show how to use location encoding to handle complex spatial data models . 
%Next, we will discuss the usage of location encoding in different scientific fields and research areas.

%In the previous section, we discuss how to utilize location encoding to handling complex spatial data models as well as how to encode spatial relations among points. 

To further show the flexibility and generalizability of location encoding, 
%As we discussed in Section \ref{def:locenc} and \ref{sec:review}, all location encoders shown in Table \ref{tab:review} are inductive learning based and task agnostic. This indicates that location encoding has a wide application area as long as the underlining spatial dataset is in the form of point sets. Section \ref{sec:complex-geo} further extends the application of location encoding to other spatial data models such as polylines, polygons, graphs, and rasters. This reflects the flexibility and generalizability of location encoding. 
this section will discuss its possible applications %of location encoding 
in different research domains. %Applications include but not limit to point cloud mapping, human mobility and urban studies, biodiversity and species distribution modeling, geospatial semantics, and climate science.
%In some research domains, location encoding are already widely accepted as an interesting research direction, while in other domain the application is almost unknown. 


\subsection{Point cloud based mapping and recognition} \label{sec:auto-drive}
%Autonomous driving or self-driving vehicle techniques are among the most cutting edge technologies in the AI field. 
%One obvious usage of location encoding in autonomous driving is LiDAR 3D point cloud mapping. 
Point cloud based mapping and recognition are among the most important usage of location encoding which is essential for many real-world applications such as autonomous navigation \citep{geiger2012we}, housekeeping robots \citep{oh2002development}, argumented/virtual reality \citep{park2008multiple}, automated indoor mapping \citep{huitl2012tumindoor}, face detection (e.g., iPhone's face ID feature), and so on. Many $\enc^{(\mP)}(\bx)$ we discussed in Section \ref{sec:review} such as PointNet, VoxelNet, and PointCNN are originally proposed for
% As we have shown before, location encoding techniques have been successfully utilized for different 
point cloud based tasks including point cloud classification and segmentation \citep{qi2017pointnet,qi2017pointnet++}, point cloud based 3D object recognition \citep{zhou2018voxelnet}, and point cloud generation \citep{achlioptas2018learning,valsesia2018learning}. 

%Despite to these success\reviseone{es}, 
\reviseone{Despite these success stories,} there are multiple challenges %still needed 
to be solved in this domain. Typical point clouds obtained from LiDAR contain 100k+ points which results in high computation and memory requirements %when training these  point-based architectures
\citep{zhou2018voxelnet}. How to scale up %these 3D feature learning 
current models to an order of magnitudes of the real-world point clouds % data sets 
while preserving the ability to capture fine-grained localized features is challenging. %an important challenge to be solve. 
Moreover, the current point-based networks %for different point cloud tasks 
usually resort to expensive neighbor searching mechanism such as KNN %k nearest neighbor 
search. % and buffer search. 
This significantly impact\reviseone{s} model efficiency. %of the models. 
How to design %the neighborhood function 
$\neifunc(\bx)$ for a more efficient neighborhood search is worth further investigation \citep{guo2020deep}.

\subsection{Human mobility and urban studies} \label{sec:mobility}
Human mobility is another important application area %of location encoding as there have been 
given the increasingly large-scale mobility data generated %and shared for social good applications
from location-based services \citep{dodge2020progress}.  %Trajectories, as one type of sequential location data, are a typical representation of human movements. Thus, it is intuitive to think about how location encoding can be applied in human mobility research just as the discussion of polyline data in Section \ref{sec:line}. 
Section \ref{sec:line} has discussed how to encode trajectories as polylines into an embedding space
%In fact, location encoding has been successfully applied to several human mobility 
for several applications such as trajectory prediction \citep{xu2018encoding} and trajectory synthesis \citep{rao2020lstm}. Moreover, location encoding is useful to understand the urban spatial structure and urban dynamics. Possible applications are place representation learning \citep{yan2017itdl,liu2019place}, urban zone representation learning \citep{zhai2019beyond,fu2019efficient}, place characteristic prediction \citep{zhu2020understanding}, and urban traffic forecasting \citep{li2017diffusion,cai2020traffic}.


\subsection{Biodiversity and species spatiotemporal distribution modeling} \label{sec:spes}
%As the study of 
%\deleted{
%\mbox{\citet{myers2000biodiversity}} showed that ``as many as 44\% of all species of vascular plants and 35\% of all species in four vertebrate groups are confined to 25 hotspots comprising only 1.4\% of the land surface of the Earth”. %This indicates the importance of these endemic species for the biodiversity of our whole ecosystem. 
%This indicates that estimating the spatiotemporal distributions of different species, especially endemic species, is the first step toward protecting biodiversity \mbox{\citep{myers2000biodiversity,marchese2015biodiversity}}. }
\revisetwo{Traditionally}, the study of species spatiotemporal distribution modeling (SDM) \citep{zuo2008geosvm} is limited to a small spatial scale due to the lack of species occurrence data. This also prohibits the usage of deep learning models on this topic. % since they usually require large amount of training samples. 
%Recently, great efforts have been putted to construct large-scale species occurrence data sets. Multiple data sets have been established 
Recently, multiple large-scale species occurrence data sets have been constructed 
such as iNaturalist dataset\footnote{\url{https://www.inaturalist.org/projects/city-nature-challenge-2020}} \citep{van2018inaturalist}, %and challenge series 
Global Biodiversity Information Facility (GBIF) dataset \footnote{\url{https://www.gbif.org/}}, Pl@ntNet dataset\footnote{\url{https://plantnet.org/en/}}, and GeoLifeCLEF Dataset\footnote{\url{https://www.imageclef.org/GeoLifeCLEF2020}} \citep{cole2020geolifeclef}. %and challenge series , and so on. 
These datasets \reviseone{accelerate} %\deleted{facilitate} 
the development of many location encoders for geo-aware species fine-grain recognition and SDM \citep{chu2019geo,mac2019presence,mai2020multi}. This will be an interesting application area for location encoding models.


\subsection{Geospatial semantics} \label{sec:geo-sem}
Geospatial semantics \citep{kuhn2005geospatial,janowicz2012geospatial} is about ``understanding GIS contents, and capturing this understanding in formal theories''. %It is a research area combining GIScience, spatial database, cognitive science, natural language processing (NLP), Artificial Intelligence (AI), and the Semantic Web \citep{janowicz2012geospatial}. 
\citet{hu2017geospatial} further divided this definition into two parts: understanding and formalization. The first part is mainly about human cognition of geographic concepts and natural language understanding of geospatial related text contents. Important applications include toponym recognition and disambiguation \citep{delozier2015gazetteer,ju2016things, wallgrun2018geocorpora,wang2020neurotpr}, text geolocalization \citep{wing2011simple,izbicki2019geolocating}, spatial relation extraction \citep{ramalho2018encoding}, geographic information retrieval \citep{purves2011geographic,janowicz2011semantics,hu2015metadata,jiang2018towards,mai2020semantically}, and text based geographic question answering \citep{chen2014parameterized}. The second part focuses on capturing this understanding through formal theories such as ontologies. Important applications include geo-ontology engineering \citep{janowicz2012observation,calegari2016supporting}, geographic knowledge graph construction \citep{regalia2019computing} and entity alignment \citep{trisedya2019entity}, and geo-ontology matching \citep{delgado2013evaluation,zhu2016spatial}. Many applications \reviseone{rely} on both understanding and formalization such as geo-analytical QA \citep{scheider2020geo,xu2020extracting},  thematic signature learning for geographic feature types \citep{adams2015thematic}, GeoKG based geographic QA \citep{mai2019relaxing,mai2020se}, and geographic knowledge graph summarization \citep{yan2019spatially}.

Location encoding can be utilized in many %of the 
tasks discussed above. For example, it can be directly used for multiple %geographic knowledge graph 
GeoKG based tasks (e.g., summarization, alignment, geo-ontology matching) to encode the spatial footprints of each geographic entities by following the idea we discussed in Section \ref{sec:graph}. %\citep{mai2020se} have utilized this idea to do knowledge graph-based geographic question answering. In a similar way, location encoding can be employed to enhance tasks in geographic knowledge graphs summarization, geographic entity alignment, and geo-ontology matching. 
For place name disambiguation, location encoding can be used to capture the correspondence between places' locations and their semantic context (e.g., place description). It can learn
%location encoding can be utilized to encode the location of each place candidate. By training the location embedding of each place with their corresponding semantic context (e.g., the description of this place), we can learn 
a spatial distribution of thematic topics over the world which serve as a prior knowledge for %place name disambiguation %, similar to the thematic signature idea proposed by 
this task \citep{ju2016things}.

%For example, in the task of toponym disambiguation, location encoding can help capture the semantics of different locations by encoding various geographic contextual information, such as elevation, climate, landmarks, and culture. These various types of contextual information specific to a location will be encoded as vector representations that can then be used as input for neural network models. In a similar way, location encoding can be employed to enhance tasks in   %both parts as long as locations are involved as parts of their inputs such as place name disambiguation, 
%geographic knowledge graphs summarization, geographic entity alignment, geo-ontology matching, and knowledge graph based geographic question answering. 
%Location encoding can also As for the other 
As for other tasks such as text geolocalization, locations are used as the model output rather than input. %he outputs of models  
For these tasks, %whether location encoding can enhance their existing model architectures and 
how location encoding can be included into the existing model design %are still research questions that 
still needs to be examined in future research.


\subsection{Climate science} \label{sec:climate}
% \deleted{Climate science %, as a subfield of physical geography, 
% is the scientific study of the weather conditions averaged over a period of time.} 
%Climate science usually includes aspects from oceanography to understand the global atmospheric water cycle\footnote{\url{https://www.usgs.gov/special-topic/water-science-school/science/atmosphere-and-water-cycle?qt-science_center_objects=0\#qt-science_center_objects}}. Global worming and weather forecasting \citep{cantelaube2005seasonal} are among the most important research topics in climate science. 
Since understanding the \reviseone{underlying} mechanism behind the important weather phenomena is the major objective of climate science, deep learning technologies is not widely used in this domain given its limited ability for model interpretation. Nevertheless, we \reviseone{see an}
%\deleted{seen}
 increasing number of \reviseone{studies which} %\deleted{study who} 
 utilize %machine learning and 
deep learning models for different prediction tasks on climate such as precipitation forecasting \citep{agrawal2019machine}, El Niño-Southern Oscillation (ENSO) forecasting \citep{ham2019deep}, weather model downscaling \citep{sachindra2018statistical}, and drought prediction \citep{agana2017deep,kaur2020deep}. Location encoding can be useful in these tasks when the \reviseone{underlying} 
%\deleted{underlining} 
datasets use %are in %irregular spatial structures 
vector data models
such as the SST %sea surface temperature 
data collected from buoys \footnote{\url{https://www.ndbc.noaa.gov/}} and the weather condition data collected from weather balloons. 



%Applications:
%\begin{enumerate}
%    \item Biodiversity hotspot prediction
%    \item Geospatial semantics: toponym recognition, geographic knowledge graphs, geographic question answering, geographic entity alignment
%    \item human mobility and trajectory prediction
%    \item weather forecasting and climate change
%    \item Epidemic forecasting????
%    \item oceanography ????
%\end{enumerate}

==> future.tex <==
% % \section{What problems remains to be solved for Location Encoding?}  
% \section{Conclusion and Vision for Future Work}
% \label{sec:future}

% In this work, we comprehensively discuss the concept of location encoding, an inductive learning based, task agnostic encoding technique for geographic locations. We advocate the idea that location encoding is a fundamental component for GeoAI research. We demonstrate the necessity of location encoding for GeoAI from two perspectives: machine learning and neuroscience perspective. A general framework has been provided to understand the current landscape of location encoding research (See Tabel \ref{tab:review}). We classify the existing location encoders into two categories - single point location encoder $\enc(\bx)$ and aggregation location encoder $\enc^{(\mP)}(\bx)$ - and we compare them from different aspects. Furthermore, we have demonstrated the possible usage of location encoding for different spatial data models and concepts as well as its applications in different domains. %. To show the generalizibility of location encoding, many potential application domains of location encoding have been discussed. 
% % In the end, we point out some challenges and future research directions. % for location encoding.
% % In this section, we list some interesting future research directions of location encoding:
% There are several interesting future research directions of location encoding:
% \begin{enumerate}
% 	\item \textbf{Region representation learning}: As we discussed in Section \ref{sec:polygon}, there are no existing method for fine-grained polygon geometry encoding (so called region representation learning) %that can encode the whole geometry of a region (e.g., a polygon or multipolygons) into a high dimensional embedding despite the fact that this region representation will be 
% 	which will be very useful in multiple tasks such as geographic entity alignment and topological relation reasoning. %In contrast to the process of encoding a polyline which can be just encoding an ordered sequence of points, the encoding result of a polygon should represent all points within this polygon which are infinite and unordered. The region representation learning framework should take this into account during model design.
% 	How to encode a polygon in an embedding space which can represent all the infinite and unordered points within it is an interesting future research direction for GIScientists. 
	
	
% 	\item \textbf{Spatiotemporal point encoding}: All location encoding methods we discussed is purely focused on location information whereas the temporal perspective is also very important. In some tasks, temporal information can be captured by a separated RNN model if a temporal sequence of these locations can be found such as trajectories. As for a set of points associated with time stamps such as species occurances, a temporal encoding model is in need which can capture temporal continuity and periodicity \citep{kazemi2019time2vec,cai2020traffic}. Moreover, how to combine location encoding with temporal encoding also needs to be investigated.
	
% 	%Given a spatiotemporal point such as one trajectory point, how to encoding the temporal information which can take into account temporal continuity and periodicity \citep{cai2020traffic}? how to combine the temporal encoding result with location encoding result? You may argue that feeding the location embeddings into a RNN model as we discussed in polyline encoding (Section \ref{sec:line}) has already accounted for the temporal information. However, this will only work for sequential data with regular time intervals. What if the time intervals become irregular as what we encounter in real world? What if the data is not in sequence structure such as a set of species occurrences? This is also an interesting research direction to be explored.
	
% 	\item \textbf{Spherical location encoding}: As we discussed in Section \ref{sec:raster}, currently, there are no existing location encoder which can preserve spherical surface distance. %take into account the spherical geometry of Earth. In other words, 
% 	When we are dealing with large-scale geospatial data sets (e.g., global SST data, species occurrences all over the world) %, large-scale species migration trajectories, and so on) 
% 	in which the map distortion problem is no longer negligible, %we have to design 
% 	a spherical-aware location encoder is required which enable us to directly \textit{calculate on a round planet} \citep{chrisman2017calculating}.
	
	
% 	\item \textbf{Unsupervised learning based location encoding}: Most of the location encoders listed in Table \ref{tab:review} are trained in a supervised learning fashion which prohibits the application of the trained location embedding on other tasks. In contrast, text encoding method such as Word2Vec, BERT are trained in an unsupervised learning manner so that the pretrained model can be utilized in different downstream tasks \citep{devlin2018bert}. %This is in fact the very reason for the popularity of these text encoding models. 
% 	How to design an unsupervised learning framework for location encoding such that the learned location embedding can be applied on multiple tasks is a very attractive research direction. Recently, multiple point cloud generative models have been proposed such as r-GAN \citep{achlioptas2018learning}, l-GAN \citep{achlioptas2018learning}, Graph-Conv GAN \citep{valsesia2018learning}, tree-GAN \citep{shu20193d}, point clould GAN \citep{li2018point}, Spectral-GAN \citep{ramasinghe2019spectral}, PointFlow \citep{yang2019pointflow}, and Generative PointNet \citep{xie2020generative}. Their objective is to generate synthetic point clouds whose probability measures are as close as possible to those of the real point clouds \citep{shu20193d}. This presents one possible unsupervised learning objective for location encoding which specifically focuses on unmarked point patterns (points without attributes). Another interesting research direction is to design an unsupervised learning framework for marked point patterns (points with attributed) which can learn the spatial distribution of point attributes. %instead of the distribution of points.
% \end{enumerate}


% %Issues:
% %\begin{enumerate}
% %    \item map projection distortion
% %    \item how to handle extreme points in attention mechanisms for spatial interpolation problem
% %    \item how to do unsupervised learning for location modeling: generative model
% %    \item how to consider long- and short-distance dependency in neural network architectures
% %    \item word embedding -> paragraph embedding; location embedding -> region embedding
% %\end{enumerate}
% %
% %
% %\textbf{r-GAN}. \citet{achlioptas2018learning} proposed multiple generative models for 3D point clouds based on AutoEncoder (AE) \citep{rumelhart1986learning}, Generative Adversarial Networks (GAN) \citep{goodfellow2014generative}, or Gaussian Mixture Model (GMM) \citep{dempster1977maximum} - AE-EMD, AE-CD, r-GAN, l-GAN, l-WGAN, and GMM. Interestingly, PointNet architecture has been utilized as the encoder module of the AutoEncoder based generative model. More specifically, Equation \ref{equ:pointnet_1} is used to independently encoder 


% \textbf{Data and Codes Availability Statement}

% There are no code implementation for this review paper.


==> spa_rel.tex <==
\section{\deleted{Relative spatial relation encoding}}   \label{sec:spa-rel}

\deleted{
All location encoders listed in Section \ref{sec:review} focus on modeling the location information of each point. %While the single point location encoders $\enc(\bx)$ purely target at encoding $\bx$, the aggregation location encoders $\enc^{\mP}(\bx)$ additionally consider the spatial context information of the center location $\bx$, i.e., $ \forall \bx_i \in \neifunc(\bx)$. However, most aggregation location encoders listed in Table \ref{tab:review} ignore the pairwise spatial relation, i.e., $\Delta \bx$, during their neighborhood aggregation $\aggfunc_{\bx_i \in \neifunc(\bx)}()$. Instead, they use $\maxpool()$ function to jointly aggregate the whole neighborhood. 
However, sometimes instead of modeling the global locations, we are more interested in modeling relative spatial relations among different objects, i.e., $\Delta \bx$. Some $\enc^{(\mP)}(\bx)$ also consider spatial relations. For example, instead of treating each $\bx_i \in \neifunc^{(\kthagglayer)}_{\knn}(\bx)$ equally during neighborhood aggregation as PointNet does, Graph-Conv GAN$^*$ uses a spatial relation specific transformation matrix $F^{(\kthagglayer)} (\locemb^{(\kthagglayer-1)}_{\bx_i} - \locemb^{(\kthagglayer-1)}_{\bx}) $ for each $\locemb^{(\kthagglayer-1)}_{\bx_i}$ to do neighborhood aggregation. In this work, we argue that by encoding the pairwise spatial relations between $\bx$ and  $\forall \bx_i \in \neifunc(\bx)$, i.e., relative spatial relation encoding, the full spatial layout of $\bx$'s spatial context is encoded in the model which makes the model more expressive.
}

% One exception is Graph-Conv GAN$^*$, which considers the pairwise spatial relation by feeding the spatial affinity $\locemb^{(\kthagglayer-1)}_{\bx_i} - \locemb^{(\kthagglayer-1)}_{\bx}$ in the location embedding space into $F^{(\kthagglayer)}_{\mathbf{w}^{(\kthagglayer)}}()$ to regress a transformation matrix $F^{(\kthagglayer)}_{\mathbf{w}^{(\kthagglayer)}}(\locemb^{(\kthagglayer-1)}_{\bx_i} - \locemb^{(\kthagglayer-1)}_{\bx}) \in \Real^{\embdim^{(\kthagglayer)} \times \embdim^{(\kthagglayer-1)}}$ for the emebdding of each neighboring location $ \locemb^{(\kthagglayer-1)}_{\bx_i}$ (See Equation \ref{equ:gc-gan_2}). We argue that \textit{by encoding the pairwise spatial relations between $\bx$ and  $\forall \bx_i \in \neifunc(\bx)$, i.e., spatial relation encoding, the full spatial layout of $\bx$'s spatial context is encoded in the model which makes the model more expressive}.



\deleted{
In fact, modeling relative spatial relations among different places %or locations 
goes to the core of many geospatial prediction tasks. % such as spatial interpolation and spatial clustering. 
For example, in many spatial interpolation models such as inverse distance weighting (IDW) \mbox{\citep{shepard1968two}}, ordinary kriging \mbox{\citep{cressie1990origins}}, the pairwise spatial relations (e.g., distance) are %explicitly 
utilized to predict the attribute values of unknown locations. %(e.g., precipitation, elevation, mineral content). %given its nearby locations and their associated attribute values. 
Pairwise distances are also essential for spatial clustering such as DBSCAN \mbox{\citep{ester1996density}}.
If the isotropic assumption is not held, direction information should also be considered. % except for distance. 
Anisotropic kriging \mbox{\citep{eriksson2000understanding}} and ADCN \mbox{\citep{mai2018adcn}} were developed as the anisotropic counterpart of ordinary kriging and DBSCAN correspondingly.
%Anisotropic kriging \citep{eriksson2000understanding} is developed based on this motivation. The same reason also motivates the development of ADCN \citep{mai2018adcn} as the anisotropic counterpart of DBSCAN for density-based clustering. 
In short, considering $\Delta \bx$ including both distance and direction information is essential for many geospatial prediction tasks.
}



\deleted{
Interestingly, many pioneering research has explored how to capture spatial relation $\Delta \bx$ among points into neural network architectures. Most of them proposed to capture only the relative distance information %spatial proximity 
among points in a point set $\mP$ by converting $\mP$ into a spatial graph (kth nearest neighbor spatial graph) in which nodes indicate points while edges are associated with pairwise distance based weights %which are computed based on pairwise distances between the involving points 
\mbox{\citep{lin2018exploiting,yan2019graph,zhu2020understanding,apple2020kriging,wu2020kriging}}. After this conversion, a GNN %graph neural network 
model %\citep{kipf2017semi,battaglia2018relational,wu2020comprehensive} 
can be applied on this spatial graph so that node attribute prediction can be done based on not only node's own features but also its spatial context. % thanks to the explicit graph structure. 
This practice has been adopted to develop NN models for multiple geospatial tasks including air quality forecasting \mbox{\citep{lin2018exploiting}}, building pattern classification \mbox{\citep{yan2019graph}}, place characteristics prediction \mbox{\citep{zhu2020understanding}}, GeoNames entity embedding learning \mbox{\citep{kejriwal2017neural}} and different spatial interpolation problems \mbox{\citep{apple2020kriging,wu2020kriging}}. %in which each node represents air quality monitoring station, a building, a place, a GeoNames entity, or a sampled location for some measurement (e.g., precipitation). More interestingly, \citet{apple2020kriging} argued that their proposed Kriging Convolutional Networks (KCN) is a neural network model which combines the advantages of GNN and kriding. 
}


\deleted{
We argue that this kind of distance weighted graph method is insufficient to capture the relative spatial relations, since this practice necessarily forfeits information about the spatial layout of points and 
%Although the converted graph structure emphasize the spatial proximity between points by using the distance based edge weights, 
some important spatial information is lost %including the original point positions %information, 
such as the cardinal direction relations \mbox{\citep{zhu2019making}} % among points, although some of these information 
which are important for some tasks \textit{when isotropic assumption is not held}. 
For instance, the cardinal direction between two air quality monitoring stations is essential for air pollution monitoring since the global wind direction will affect the diffusion speed of the air pollution in different directions. 
}

%Instead of using distance based edge weight method, we propose two approaches to incorporate spatial information into the graph encoding process: 1) \textit{node location encoding}: using the location encoder as the node embedding encoder (or one component of it) to fully capture the location information of each node; 2) \textit{spatial relation encoding}: using a location encoder to encode the spatial relation $\Delta \bx$ between two nodes and utilizing $\enc(\Delta \bx)$ in node neighborhood aggregation step.

%The idea of node location encoding is to use one kind of single point location encoders in Table \ref{tab:review} as the node embedding encoder or one component of it. The location embedding can be seen as the initial node embedding for each node. Then any kind of graph neural networks can be applied on top of it to do message passing among different nodes. \citet{mai2020se} has used this kind of idea. They utilized the $\theory$ location encoder as one component of entity encoder (node embedding encoder). Then a knowledge graph embedding training objective is applied on top it and the whole model is trained end-to-end. As for encoding point sets, instead of use the distance weighted graph methods as \citet{lin2018exploiting,yan2019graph,zhu2020understanding,apple2020kriging,wu2020kriging}, we can directly use our aggregation location encoder framework proposed in Equation \ref{equ:aggenc}. 


\deleted{
Instead, we advocate the idea of \textit{relative spatial relation encoding} $\enc(\Delta \bx)$ which encodes the pairwise spatial relationship %between two node
%, i.e., 
$\Delta \bx$, into an embedding space by a location encoder. %The result 
$\enc(\Delta \bx)$ %encodes the spatial affinity between two points which 
can be used during the neighborhood aggregation step. %Equation \ref{equ:gc-gan_2} shows how Graph-Conv GAN$^*$ uses spatial relation encoding in the neighborhood aggregation step. 
%Note that Graph-Conv GAN and Graph-Conv GAN$^*$ are utilized in the context of point cloud generation and segmentation task while the locations of points and their spatial relationship are the main features for the tasks. We call the underlining datasets \text{unmarked spatial point patterns}. In other tasks involving \textit{marked spatial point patterns} such as multiple spatial interpolation tasks where we are interested predicting the attribute value of unknown locations, we may not need to encode the locations of the location of each observation. Instead, we encode the spatial relations among them. 
Graph-Conv GAN$^*$ adopts this idea by considering both spatial relation and global position information (See Equation \ref{equ:gc-gan_2}). Sometimes, we can ignore the global position information and focus on spatial relation encoding. 
\mbox{\citet{mai2020multi}} proposed an example of these models by incorporating $\enc(\Delta \bx)$ into a graph attention network (GAT) architecture. 
We generalize their idea and summarize it as Equation \ref{equ:spa-rel-enc}. %Here, we assume we have a marked 
Given a point set $\mP=\{\pt_i\}$ where each point $\pt = (\bx, \bv)$ is associated with its location $\bx$ and attribute $\bv$. $\neifunc(\pt)$ is $\pt$'s spatial neighborhood.
Similar to $\enc^{(\mP)}(\bx)$, %our aggregation location encoder (Equation \ref{equ:aggenc}),
\mbox{\citet{mai2020multi}} also uses $\numagglayer$ aggregation layers. 
The initial point embedding is computed purely based on $\bv$ %its feature information 
as shown in Equation \ref{equ:spa-rel-enc_1} where $\feenc()$ is the feature encoder. %This means the location information is not used by the node embedding encoder which is different from the node location encoding method. 
The spatial relationships $\Delta \bx_j = \bx - \bx_{j}$ between %the center point 
$\pt$ and %all of its neighbors 
$\forall \pt_{j} \in \neifunc(\pt)$ are utilized in the neighborhood aggregation step as shown in Equation \ref{equ:spa-rel-enc_2}-\ref{equ:spa-rel-enc_4}. %$\neifunc(\node)$ is the graph neighborhood of node $\node$ which can simply be all nodes directly connected with $\node$ by edges. 
% $\pt_{j} \in \neifunc(\pt)$ is one of its neighboring node where $\bx_j$ and $\bv_j$ is the location and feature of $\pt_{j}$. 
Equation \ref{equ:spa-rel-enc_2} shows how to do neighborhood aggregation based on a self-attention mechanism as GAT \mbox{\citep{velivckovic2018graph}} where $\attnsize$ is the total number of attention heads. $\locemb^{(\kthagglayer-1)}_{\bv_{j}}$ is the \textit{feature embedding} of point $\pt_j$ at the $\kthagglayer-1$-th layer. $\attnscr_{j \attnidx}$ is its attention score which is normalized %which is a normalized score based on the raw attention score $\sigma_{j\attnidx}$  
across $\neifunc(\pt)$ % by a softmax function 
(See Equation \ref{equ:spa-rel-enc_3}).
% Equation \ref{equ:spa-rel-enc_4} indicates that 
$\enc(\bx - \bx_{j})$ is utilized in the attention score computation so %the spatial affinity 
$\Delta \bx_j = \bx - \bx_{j}$ %between $\pt$ and $\pt_j$ 
is considered in the aggregation step where $\attnvec_{\attnidx}$ is a learnable attention vector for the $\attnidx$th attention head (See Equation \ref{equ:spa-rel-enc_4}).
}




{\color{blue}
	Equation deleted
\begin{subequations}
    \vspace{-0.8cm}
	\label{equ:spa-rel-enc}
	\begin{align}
	\locemb^{(0)}_{\bv} & = \feenc(\bv), \label{equ:spa-rel-enc_1} \\	
	\locemb^{(\kthagglayer)}_{\bv} & = \attnact(\dfrac{1}{\attnsize} \sum_{\attnidx=1}^{\attnsize} \sum_{\pt_{j} \in \neifunc(\pt)} \attnscr_{j \attnidx}\locemb^{(\kthagglayer-1)}_{\bv_{j}}) , \label{equ:spa-rel-enc_2} \\
	where \; \attnscr_{j \attnidx} & =  \frac{exp(\sigma_{j\attnidx})}{\sum_{\pt_{o} \in \neifunc(\pt)} exp(\sigma_{o\attnidx})} , \label{equ:spa-rel-enc_3} \\
	\sigma_{j\attnidx} & = \leakyrelu(\attnvec_{\attnidx}^{T}[\locemb^{(\kthagglayer-1)}_{\bv}; \locemb^{(\kthagglayer-1)}_{\bv_{j}};\enc(\bx - \bx_{j}) ]). \label{equ:spa-rel-enc_4}
 	\end{align}
\end{subequations}
}


